Real-Time Line-Based Room Segmentation and Continuous Euclidean Distance Fields

Continuous maps representations, as opposed to traditional discrete ones such as grid maps, have been gaining traction in the research community. However, current approaches still suffer from high computation costs, making them unable to be used in large environments without sacrificing precision. In this paper, a scalable method building upon Gaussian Process-based Euclidean Distance Fields (GP-EDFs) is proposed. By leveraging structure inherent to indoor environments, namely walls and rooms, we achieve an accurate continuous map representation that is fast enough to be updated and used in real-time. This is possible thanks to a novel line-based room segmentation algorithm, enabling the creation of smaller local GP-EDFs for each room, which in turn also use line segments as its shape priors, thus representing the map more efficiently with fewer data points. We evaluate this method in simulation experiments, and make the code available open-source.

==> Sections/prelim.tex <==
\section{Preliminaries}
\subsection{Euclidean Distance Fields}\label{subsec:edf}
Given a subset $\Omega \subset \mathbb{R}^n$, with its boundary denoted as $\partial \Omega$, an Euclidean distance field (EDF) provides the shortest Euclidean distance from a point $\bm{x} \in \Omega$ to $\partial \Omega$, represented as $d(\bm{x})$. The EDF can be mathematically expressed as follows~\cite{wu_faithful_2021}:
%
\begin{equation}
d(\bm{x}) = \min_{\bm{y} \in \partial \Omega}||\bm{x} - \bm{y}||.
\end{equation}

Furthermore, according to~\cite{mauch2000fast}, the gradient of a continuous EDF satisifes the Eikonal equation, which is given by:
\begin{equation}
    ||\nabla d(\bm{x})|| = 1 \; \; \; \; \; \bm{x} \in \mathbb{R}^n,
\end{equation}
with the boundary constraint $d(\bm{x}) = 0$ for all $\bm{x} \in \partial \Omega$.

\subsection{Gaussian Process Regression}
%Gaussian process regression, as described in \cite{rasmussen_gaussian_2006}, is a non-parametric, Bayesian approach for solving regression problems. It is based on the assumption that the target function $f$ is drawn from a Gaussian process, conceptually understood as a distribution over an infinite number of possible functions.

A Gaussian process $\mathcal{GP}$ is fully defined by its mean function $m(\bm{x})$ and covariance function $k(\bm{x},\bm{x'})$, and can formally be expressed as~\cite{rasmussen_gaussian_2006}:
\begin{equation}
f(\bm{x}) \sim \mathcal{GP}(m(\bm{x}), k(\bm{x}, \bm{x'})).
\end{equation}

A data set of $N$ (noisy) sensor measurements is given by $\mathcal{D}~=~\{x_i,y(x_i)\}^N_{i=1}$, with $x_i \in \Real^n$ and $y(x_i) = f(x_i) + \epsilon$, where $\epsilon \sim \mathcal{N}(0, \sigma^2)$ is zero-mean additive sensor noise. The posterior belief of $f$ at a position $x^*$, conditioned on the data set $\mathcal{D}$, is given by $f(x^*) \mid \mathcal{D} \sim \mathcal{N}(\bar{f}(x^*), \mathbb{V}[f(x^*)])$ where
%
\begin{align}
    \bar{f}(x^*) &= \mathbf{\kappa}(x^*)^T (\bar{K} + \sigma_n^2 I)^{-1} \mathbf{y} \label{eq:gpmean}\\
    \mathbb{V}[f(x^*)] &= \kappa(x^*,x^*) - \mathbf{\kappa}(x^*)^T (\bar{K} + \sigma_n^2 I)^{-1} \mathbf{\kappa}(x^*). \label{eq:gpvar}
\end{align}
%
with $\mathbf{y} = [y(x_1), \dots, y(x_N)]^T$, $\bar{K} \in \Real^{N \times N}$ a positive definite matrix with $\bar{K}[i,j] = \kappa(x_i,x_j)$, and $\mathbf{\kappa}(x^*) = [\kappa(x_1,x^*), \dots, \kappa(x_N,x^*)]^T$.


% In the Gaussian process prior, we incorporate our initial knowledge about the target function $f$ using the mean function $m(\bm{x})$ and covariance function $k(\bm{x},\bm{x'})$. While the mean function is often set to zero for simplicity, it can also mirror initial knowledge about the characteristics of the data and the function under consideration.

% Upon gathering the noisy observations $\bm{y}$, the prior is updated to yield a posterior distribution over functions. This update takes place by conditioning the Gaussian process prior on the observed data, leading to a Gaussian process posterior $p(f|\bm{y})$. This posterior is itself a Gaussian process and reflects an updated set of plausible functions that align with the data. It possesses a new mean and covariance function, derived from the prior and the observed data.

% After determining the Gaussian process posterior $p(f|\bm{y})$, it can be used to make predictions at previously unseen data points. This involves calculating the predictive distribution at a new point $\bm{x^*}$, which is computed based on the mean and variance of the posterior Gaussian process at that point. As a result, the predictive distribution not only provides the most probable function value (the mean) at $\bm{x^*}$, but also a measure of uncertainty (the variance).

% \subsubsection{Sparse Variational Approximation}
% Numerous sparse approximations have been devised to address the $O(N^3)$ computation complexity of exact Gaussian process regression. Variational inference is used in~\cite{pmlr_v5_titsias09a} in an attempt to minimize the divergence between the approximate and the original GPs.

% The approximation strategy introduces a variational distribution over the function values, exemplified as a multivariate Gaussian, denoted as $q(f) = \mathcal{N}(m, S)$. The approximate posterior is parameterized by a set of $M \ll N$ inducing variables $\bm{u}$ evaluated at inducing locations $Z$, which form a subset of the function values $f={f_{\neq \bm{u}}, \bm{u}}$, and aims to summarize the data.

% Thus, the approximate posterior is modeled as $q(f) = p(f_{\neq \bm{u}}|\bm{u})q(\bm{u})$, where $q(\bm{u})$ signifies a variational distribution over $\bm{u}$ and $p(f_{\neq \bm{u}}|\bm{u})$ represents the prior distribution of the remaining function values. The variational parameters are chosen to minimize the distance between the variational approximation $q(f)$ and the exact posterior $p(f|\bm{y})$ by maximizing a variational lower bound on the true marginal likelihood $p(\bm{y})$. This method notably diminishes the computational complexity of predictions from $\mathcal{O}(N^2)$ to a manageable $\mathcal{O}(M^2)$.

\subsubsection{Streaming Sparse GPs}
In~\cite{bui_streaming_2017}, an online approach to sparse variational approximation of GPs is introduced. The approach allows for online updating of the model using incoming new data points while keeping the computational cost manageable. The model works on the principle of sequentially arriving data, where new data points $\bm{y}_{new}$ are added to the dataset $\bm{y}_{old}$ at each step.

At every step, it approximates both the marginal likelihood $p(\bm{y})$ and the posterior $p(f|\bm{y})$, which can be utilized for real-time prediction. As the model operates in an online mode, only the most current data points $\bm{y}_{new}$ are directly accessible due to computational restrictions, such as memory limitations. The impact of the previous data on the current posterior needs to be transferred through the previous posterior.

The model achieves this by formulating a sparse variational free energy approximation which summarizes the old data using inducing points. When incorporating new data points, the model employs an approximation of the true posterior from the preceding step, represented as $q_{old}(f)$. This needs to be updated to the new approximation, $q_{new}(f)$, using a variational update that refines the distribution to a manageable form using the inducing points. As new regions of the input space are revealed with time, the model adjusts the positions of these inducing points accordingly.

Suppose we define $a = f(z_{old})$ and $b = f(z_{new})$ as the function values at the inducing points before and after integrating new data. We can describe the previous approximate posterior as $q_{old}(f) = p(f_{\neq a}|a)q_{old}(a)$, under the assumption that $q_{old}(a) = \mathcal{N}(a; m_a, S_a)$. In a similar manner, the updated posterior approximation is denoted as, $q_{new}(f) = p(f_{\neq b}|b)q_{new}(b)$.

The optimal approximate posterior is then derived for the regression case by setting the derivative of the variational free energy with respect to $q(b)$ to zero.

\subsection{GP-EDF}
To successfully employ a Gaussian processes in the approximation of Euclidean distance fields, one must consider specific modifications to the standard Gaussian process regression. In particular, a logarithmic transformation, inspired by the heat method~\cite{crane_geodesics_2013}, is performed on the Gaussian process, which is essential for obtaining accurate distance fields. This approach also involves the use of a particular member of the Matérn family of covariance functions, as detailed in~\cite{wu_faithful_2021}. Such adaptations ensure compliance with the properties of EDFs outlined in Section~\ref{subsec:edf}.

Gaussian Process regression has been used in~\cite{wu_faithful_2021, barbosa2022risk} to build an approximation of the EDF based on a dataset of samples from the surface of the obstacles. Based on heat diffusion methods~\cite{crane_geodesics_2013}, a GP model is constructed using

With a set of measured surface points ${\bm{x}_i}$ and target values set as $y_i = 1$, the distance $d$ at a query point $\bm{x^*}$ can be determined by the following expression:
\begin{equation}
d(\bm{x^{*}}) = -\frac{\ln{\bar{f}}}{\lambda},
\end{equation}
where $\bar{f}$ represents the predictive mean at the query point $\bm{x}$. 

The Matérn family of covariance functions is formulated as follows:
\begin{equation}
k(\bm{x}, \bm{x}') = \sigma^2 \frac{2^{1-\nu}}{\Gamma(\nu)} \left( \frac{\sqrt{2\nu}|\bm{x}-\bm{x}'|}{\lambda} \right)^\nu K_\nu\left( \frac{\sqrt{2\nu}|\bm{x}-\bm{x}'|}{\lambda} \right),
\end{equation}
where $\lambda$ represents the characteristic length scale, $\sigma^2$ indicates the variance, and $K_\nu$ is the modified Bessel function of the second kind of order $\nu$. As proposed by~\cite{wu_faithful_2021}, a Matérn covariance with $\nu = 3/2$ is selected, and a large value for $\lambda$ is preferred to yield more precise EDFs.
